Parameterized Verification under TSO with Data Types

We consider parameterized verification of systems executing according to the total store ordering (TSO) semantics. The processes manipulate abstract data types over potentially infinite domains. We present a framework that translates the reachability problem for such systems to the reachability problem for register machines enriched with the given abstract data type. We use the translation to obtain tight complexity bounds for TSO-based parameterized verification over several abstract data types, such as push-down automata, ordered multi push-down automata, one-counter nets, one-counter automata, and Petri nets. We apply the framework to get complexity bounds for higher order stack and counter variants as well.

==> Figures/rules_counter.tex <==
\begin{figure}[h]
	\begin{equation*}
		\resizebox{\hsize}{!}{
			\inferencebox[$\inc$]{
			}{
				\val \step[\inc]\Counter \val+1
			}
			\quad
			\inferencebox[$\dec$]{
				\val > 0
			}{
				\val \step[\dec]\Counter \val-1
			}
			\quad
			\inferencebox[$\isZero$]{
				\val = 0
			}{
				\val \step[\isZero]\Counter \val
			}
		}
	\end{equation*}
	
	\caption{The transition relation of $\Counter$.}
	\label{fig:rules_counter}
\end{figure}

==> Figures/rules_ncounter.tex <==
\begin{figure}[h]
\begin{equation*}
	\resizebox{\hsize}{!}{
    \inference[$\inc$]{
        t(i) = a
    }{
        t \step[\inc_i]\ncounter t[i \leftarrow a+1]
    }
    \quad
    \inference[$\dec$]{
        t(i) = a > 0
    }{
        t \step[\dec_i]\ncounter t[i \leftarrow a-1]
    }
    \quad
    \inference[$\isZero$]{
        t(i) = 0
    }{
        t \step[\isZero_i]\ncounter t
    }
}
\end{equation*}

\caption{The transition relation of the $n$ counter abstract data type $\ncounter$.}
\label{fig:rules_ncounter}
\end{figure}

==> Figures/rules_stack.tex <==
\begin{figure}[h]
\begin{equation*}
    \inferencebox[$\push$]{
        \stacksymbol \cdot \word = \word'
    }{
        w \step[\push\of\stacksymbol]\stack \word'
    }
    \quad
    \inferencebox[$\pop$]{
        \word = \stacksymbol \cdot \word'
    }{
        \word \step[\pop\of\gamma]\stack \word'
    }
    \quad
    \inferencebox[$\isEmpty$]{
        \word = \emptystack
    }{
        \word \step[\isEmpty]\stack \word
    }
\end{equation*}
\caption{The transition relation of the stack abstract data type $\stack$.}
\label{fig:stack_relation}
\end{figure}
